Improving Multimodal fusion via Mutual Dependency Maximisation

Multimodal sentiment analysis is a trending area of research, and the multimodal fusion is one of its most active topic. Acknowledging humans communicate through a variety of channels (i.e visual, acoustic, linguistic), multimodal systems aim at integrating different unimodal representations into a synthetic one. So far, a consequent effort has been made on developing complex architectures allowing the fusion of these modalities. However, such systems are mainly trained by minimising simple losses such as $L_1$ or cross-entropy. In this work, we investigate unexplored penalties and propose a set of new objectives that measure the dependency between modalities. We demonstrate that our new penalties lead to a consistent improvement (up to $4.3$ on accuracy) across a large variety of state-of-the-art models on two well-known sentiment analysis datasets: \texttt{CMU-MOSI} and \texttt{CMU-MOSEI}. Our method not only achieves a new SOTA on both datasets but also produces representations that are more robust to modality drops. Finally, a by-product of our methods includes a statistical network which can be used to interpret the high dimensional representations learnt by the model.

==> coucou.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%% Study with class imbalance %%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


% Comparison f-div / kl / wasserstein (cas des machin correle gradient) // expected with the behavior (cite the fact the borne is loos )

% Comparing pretrained > not pretrained selon le papier de magbert c'est pas vrai

% KL or Wassertstein is still an open question 

% We can observe that the MAE is not a good proxy on the last task when doing prediction.=> cite the EMNLP paper
% Same with correlation =>  although we follow standart practices

% BEST improvement with TFN : how can we explain it ? Does it mean that decomposiiton in fact is the less efficient => ask for futur woek 

% MAGBERT we also observe a +1.2 improvement (think in terme of relative improvement) the MAG is simple efficient but gain at beeing coupled with our losses : ) 

% Recommendation: use the wasserstein loss ? a voir comment reformuler tout ca 



%%%%%%https://imotions.com/blog/facial-action-coding-system/?fbclid=IwAR0p-wBiI-p17NzM8ubajuD3DaHChuvWimz1bnJIo8ImnxMtBA_C-Kf1vFw

==> model_b.tex <==
\section{Problem Setting}

We have an input review $x \in \mathcal{X}$ that can be either a sentence or a video with an associated label $y \in \mathcal{Y}$.
$x$ can be decomposed in three modalities $x^t,x^a,x^v$. 
The idea is to allow a better co-learning (ensure that the system takes as input all the modalities).

\subsection{Simple Idea}
In this first idea, the underlying intuition is that we have \textbf{ONE} source that generates an input signal composed of three sub-signals. Instead of minimising the MSE we propose to minimise:

\begin{align}
\mathcal{L} &= MSE - \lambda * I((X^t,X^a,X^v);Z) \\
& \leq MSE - \lambda * I^{lower}((X^t,X^a,X^v);Z)
\end{align}
Here we take MINE :) or NCE machine

\subsection{Second Idea}
In this first idea, the underlying intuition is that we have \textbf{THREE} different sources that generate a correlated signal.

The goal is to maximimse the multivariate mutual information
\begin{align}
I(X^t,X^a,X^v,Z) &= \sum_{i=1}^{3} I(X_i, Z | X_{i-1}, \cdots, X_1)
\end{align}
This expression is not symetrical should we aim for a symetric expression ?

\begin{align*}
    I(X_i, Z | X_{i-1} \cdots X_1) &= D_{KL}(p(X_i, Z|X_{i-1} \cdots X_1) || p( Z|X_{i-1} \cdots X_1) p(X_i|X_{i-1} \cdots X_1)) \\
    & \geq \mathbb{E}_{(p(X_i, Z|X_{i-1} \cdots X_1)} \big[T\big] - \mathbb{E}_{p( Z|X_{i-1} \cdots X_1) p(X_i|X_{i-1} \cdots X_1)}\big[e^T\big]
\end{align*}
where T is a classifier function.

\subsection{Third idea: early fusion}

Total correlation $C$ between $X_1, \dots, X_n$
\begin{align*}
C(X^t,X^a,X^v,Z) &= - \mathbb{E}_{p_{X^t,X^a,X^v,Z}} \log \big[\frac{p_{X^t,X^a,X^v,Z}}{ p_{X^t}\times p_{X^a}\times p_{X^v}\times p_Z}\big] \\
&= D_{KL}(p_{X^t,X^a,X^v,Z}||p_{X^t}\times p_{X^a}\times p_{X^v}\times p(Z)) \\
& \geq \mathbb{E}_\mathbb{P} [T] - \log \mathbb{E}_\mathbb{Q} [e^T]
\end{align*}

\subsection{Fourth idea late fusion}

Total correlation $C$ between $X_1, \dots, X_n$
\begin{align*}
C(X^t,X^a,X^v) &= - \mathbb{E}_{p_{X^t,X^a,X^v}} \log \big[\frac{p_{X^t,X^a,X^v}}{ p_{X^t}\times p_{X^a}\times p_{X^v}}\big] \\
&= D_{KL}(p_{X^t,X^a,X^v,Z}||p_{X^t}\times p_{X^a}\times p_{X^v}) \\
& \geq \mathbb{E}_\mathbb{P} [T] - \log \mathbb{E}_\mathbb{Q} [e^T]
\end{align*}

